Study of event and particle selection effects on elliptic flow background at the isobar experiments based on AMPT model

Measurement of the Chiral Magnetic Effect (CME) has been a popular topic of high-energy nuclear physics in the last decade. The flow correlation $\gamma$ between charged hadron pairs of the same and opposite charges and their difference $\Delta \gamma$ were measured to separate the CME-driven signal from the collective flow background especially second-order elliptic $v_{2}$. The STAR experiment have stepped further to the isobar experiment to compare $\gamma$ and $\Delta \gamma$ between Ru+Ru and Zr+Zr ~\cite{PhysRevC.105.014901}, which were theoretically expected to produce the same elliptic flow background but different CME signals. However, the measured flow backgrounds also differ between Ru+Ru and Zr+Zr, indicating more fine-tuning of RP and centrality definition necessary. This analysis applied the AMPT model~\cite{PhysRevC.72.064901} to simulate the same collision system and energy as the STAR isobar experiment. Since the AMPT model does not include magnetic field effects, we expect comparing its output between Ru+Ru and Zr+Zr collision systems can provide an insight of the possible bias of flow background definition, and help improve the measurement of CME signal in real experiments. Multiple combinations of centrality and flow definition were chosen to study how the $v_2$ and their difference would be affected, especially by varying the particles selection of charge versus neutral properties and broadening (pseudo-)rapidity regions, while STAR CME work relied on charged-only particles at central rapidity.

==> wy_command.tex <==
\newcommand{\ruru} {Ru+Ru}
\newcommand{\zrzr} {Zr+Zr}

\newcommand{\pt}   {\ensuremath{p_\mathrm{T}}}
\newcommand{\GeV}  {Ge\kern-.1emV}
\newcommand{\gevc} {GeV/$\textsl{c}$}
\newcommand{\snn}  {\ensuremath{\sqrt{S_{\ensuremath{NN}}}}}

